Cyclotron Modeling Phase-Resolved Infrared Spectroscopy of Polars III: AM Herculis and ST Leo Minoris

We present phase-resolved low resolution infrared spectra of AM Her and ST LMi, two low-field polars that we observed with SPEX on the IRTF. Optical/NIR lightcurves are also published to help constrain the viewing geometry and brightness of the objects at the time they were observed. Currently, only limited IR spectra have been published for these objects, and none with the phase-coverage presented here. In both cases, the resulting spectra are dominated by emission from the secondary star in the NIR. However, the emission regions are also self-eclipsed, allowing us to isolate the cyclotron emission through subtraction of the dim-phase spectrum. We use a ``Constant Lambda'' prescription to model the changing cyclotron features seen in the resulting data. For AM Her, we find a best fit model of: B = 13.6 MG, kT = 4.0 keV, and logLambda = 5.0. The cyclotron derived accretion geometry is consistent with an orbital inclination of 50 degrees and a magnetic co-latitude of 85 degrees. For ST LMi, B = 12.1 MG, kT = 3.3 keV, and logLambda = 5.7 with an orbital inclination of 55 degrees and a magnetic co-latitude of 128 degrees.

==> README <==
To whom it may concern:

We would like to re-submit our paper entitled "Cyclotron Modeling 
Phase-Resolved Infrared Spectroscopy of Polars III: AM Herculis and ST Leo 
Minoris" for consideration for publication in the Astrophysical Journal. 
New Mexico State University will assume all costs associated with page charges.
As ennumerated below, we have made all of the changes recommended by the 
referee.

Sincerely,

Ryan Campbell

Astronomy Department
New Mexico State University
Box 30001/MSC 4500
1320 Frenger Street
Las Cruces, NM 88003
Ph: 505-646-4914
Fax: 505-646-1602

There are 9 figures that go along with this paper. Figures 2 & 6 are in black &
White, the rest are in color.

*******************************************************************************
Changes Made to Manuscript
*******************************************************************************
1. In Section 2, addition of references for the SPEX and SQIID instruments 
would be useful. =>

Added the references: Rayner et al.(2003) for SPEX, and Ellis et al. (1992) for
SQIID.

*******************************************************************************

2. In Section 2, for consistency and completeness, the definition of 'R' 
in '...produces R~250 spectra...' should be given. =>

Included! Now reads, R(=lambda/(delta lambda)) ~ 250.

*******************************************************************************

3. In Section 2, it would help to give a table listing the various 
observations of each object (i.e. an observation log), which includes 
dates/times/instruments of the various runs, number of spectra obtained, 
exposure times, duration of photometric observations, etc. collated in one 
place. =>

Added an observation log as new Table 1. Renamed old Table 1 => 2 and table 
2 => 3.

*******************************************************************************
4. In Section 3, I don't understand the word 'namesake' in '...and 
namesake \Lambda...' =>

I suppose that the wording is a little weird. REMOVED.


*******************************************************************************
5. In Section 3.1, the text refers to BVRIJHK observations taken on 2006 
May 20, but in Section 2 these are said to be from 2005 May 20 and in the 
caption to Figure 3, they are from 2002 May 20. I presume these are in fact 
all from the same date! =>

Good Catch! The correct date was 2005 May 20. The text has been changed to
reflect this.

*******************************************************************************
6. In Section 3.2, it is unclear why there are gaps in Fig 8b for the spectra 
of ST LMi in the 2005 extreme low state ... there are no gaps in the spectra 
from 2006 (in Fig 8a) yet these data were obtained with the same instrument 
weren't they? Please clarify. =>

Because the object was much fainter during the extreme low-state, the spectra
were very noisy and telluric correction was not possible in the regions which
have been clipped.

*******************************************************************************
7. In the 5th paragraph of Section 3.2, the i and beta values previously 
derived for ST LMi are listed for the first time. I think these should be in 
the appropriate place in Section 1, where the similar parameters for AM Her 
are listed. =>

Added the following sentence to the end of the ST LMi section of Section 1.
" The accretion geometry of the primary emission region has also been
previously determined, with 55$^{\circ}$ $\leq i \leq$ 64$^{\circ}$ and 
140$^{\circ}$ $\leq \beta \leq$ 150$^{\circ}$ (Schmidt et al., 1983; 
Potter, 2000)". I left in similar information in section 3.2 to act as a
reminder to the reader.


*******************************************************************************
8. I think Section 4 would benefit from another subsection heading to 
encompass some or all of the 5 paragraphs that precede Subsection 4.1 =>

A new subsection called "Analysis of Results" has been added.

*******************************************************************************
9. In the 4th paragraph of Section 4, the word 'both' should be deleted 
from '...WE find both the similarity of...' and the word 'infer' towards 
the end of the paragraph should I think be 'imply'. =>

Done.

*******************************************************************************
10. The caption to Fig 4 says 'no cyclotron emission was observed from \phi = 
0.31 to \phi=0.70' yet the text of the paper refers to the appropriate phase 
range as 0.27 to 0.74. Please make them consistent. =>

Phi = 0.27 to 0.74 is correct. Figure caption changed.

*******************************************************************************
11. In the caption to Fig 5, lose the word 'on' from '...SQIID on of the 
April 9' =>

Done.


*******************************************************************************

12. The caption to Fig 6 says that the zoomed part has labels 'P' and 'S' 
indicating the times of photometry and spectroscopy, but the 'P' label is 
only in the time region covered by the un-zoomed part. =>

The Fig. 6 caption now reads, "Long-term lightcurves of ST LMi. top: $V$-band 
photometry following ST LMi from late 1991 to early 2006. bottom: Zoom-in of 
the year surrounding our IRTF/SPEX spectroscopy. The ``P'' denotes the epoch 
of our photometry, while ``S'' marks our spectroscopic data during the 2005 
extreme low-state and the 2006 low-state, respectively." The new wording should
clear-up things.

*******************************************************************************
End of Comments
*******************************************************************************

